Enriching Relation Extraction with OpenIE

Relation extraction (RE) is a sub-discipline of information extraction (IE) which focuses on the prediction of a relational predicate from a natural-language input unit (such as a sentence, a clause, or even a short paragraph consisting of multiple sentences and/or clauses). Together with named-entity recognition (NER) and disambiguation (NED), RE forms the basis for many advanced IE tasks such as knowledge-base (KB) population and verification. In this work, we explore how recent approaches for open information extraction (OpenIE) may help to improve the task of RE by encoding structured information about the sentences' principal units, such as subjects, objects, verbal phrases, and adverbials, into various forms of vectorized (and hence unstructured) representations of the sentences. Our main conjecture is that the decomposition of long and possibly convoluted sentences into multiple smaller clauses via OpenIE even helps to fine-tune context-sensitive language models such as BERT (and its plethora of variants) for RE. Our experiments over two annotated corpora, KnowledgeNet and FewRel, demonstrate the improved accuracy of our enriched models compared to existing RE approaches. Our best results reach 92% and 71% of F1 score for KnowledgeNet and FewRel, respectively, proving the effectiveness of our approach on competitive benchmarks.

==> bigtext.tex <==
\section{BigText Knowledge Graph}
\label{sec:bigtext}

Our BigText project\footnote{URL hidden due to double-blind reviewing.} is driven by the strong belief that natural-language text is the most comprehensive knowledge base we can possibly have; it just needs to be made machine-accessible for further processing and analytics. 

Well-established knowledge bases (KBs), such as YAGO~\cite{suchanek2007yago}, DBpedia~\cite{auer2007dbpedia}, Freebase~\cite{bollacker2008freebase} or Wikidata~\cite{vrandevcic2014wikidata}, apply various IE techniques to capture and store facts extracted from unstructured and semi-structured  resources such as text, tables and infoboxes. They aim at a triple-based representation of knowledge reflecting the semantic relationships between pairs of real-world objects (i.e., entities and concepts). However, these approaches leave out sensible contextual information about the facts' origins, such as the documents, paragraphs and sentences, from which they have been extracted. Information retrieval (IR), on the other hand, has been very successful in efficiently operating on indexed collections of millions of documents by exploiting various context-based statistics, such as term- and document-frequencies, co-occurrences, and complex modeling approaches \cite{manning2010introduction}. These IR techniques are however still largely limited to an over-simplified ``bag of words'' representation which remains almost completely oblivious to the documents' internal structure.

\begin{figure}[!t]
  \centering
  \includegraphics[width=3.0in]{figures/BigTextGraphRepr.png}
  \caption{A snapshot of the BigText graph viewed as a corpus of interconnected documents.}
  \label{fig:BigTextDocs}
\end{figure}

With our BigText approach, we aim to combine the strengths of the two worlds of IE and IR while avoiding their conceptual simplifications. BigText represents a document collection in the form of a redundant (i.e., ``hybrid'') knowledge graph (KG) which keeps the original document structure, including the documents’ domains, hyperlinks and other metadata, intact. By including the documents’ substructures, such as natural-language sentences and their embedded clauses, as well as lists and tables, the graph gets augmented both with mentions of named entities and the syntactic and semantic dependencies that these substructures contain. Furthermore, by resolving the mentions to a canonical ground-truth set of real-world entities, a plethora of additional links among these entities and their contexts within and across the documents' boundaries can be established.
Figure~\ref{fig:BigTextDocs} shows a few snapshots of Wikipedia articles devoted to actors and movies\footnote{We use Wikipedia articles here to keep aligned with the experiments described in this paper. Note however that the choice of the document collection is not limited to any particular document type and can also combine heterogeneous natural-language resources, such as books, news, social networks, etc.}. These stand-alone documents are linked to each other via the entities they jointly mention. For example, ``American Beauty'' is one such entity that relates the three articles.

\smallskip
\noindent\textbf{Design \& Implementation.~}
BigText aims at processing large collections, consisting of millions of text documents. We currently employ Apache Spark \cite{spark:Zaharia} and its integrated distributed graph engine, GraphX \cite{GraphX:Xin}, which allows us to model the entire collection as a unified property graph that can also be distributed across multiple compute nodes or be deployed on top of any of the common cloud architectures, if desired.

\smallskip
\noindent\textbf{Property Graph.~} As depicted in Figure~\ref{fig:BigTextStruct}, our BigText graph distinguishes five types of {\em vertices}: {\em documents} ($d$), {\em sentences} ($s$), {\em clauses} ($c$) -- units of coherent information, each with an obligatory subject and a verbal or nominal predicate, and several optional (in)direct object(s), complement(s) and adverbials that further contextualize the two mandatory components, {\em mentions} ($m$), and {\em entities} ($e$). GraphX allows us to associate an extensible list of properties for each vertex type, such that the (ordered) vertices are able to losslessly (and partly even redundantly) capture all the extracted information from a preconfigured Natural Language Processing (NLP) pipeline together with the original text sources. Figure~\ref{fig:VertexProp} shows an internal representation of the property graph. For example, a document property stores the corresponding title and other relevant metadata, such as timestamp and source URL, while a mention vertex is augmented with morphological data, such as part-of-speech (POS) and lemma, syntactic role within the sentence, as well as entity-type information, where applicable. Entity vertex property carries on the result of mention disambiguation to a canonicalised entity.
\begin{figure}[!t]
  \centering
  \includegraphics[width=3.0in]{figures/Graph_Struct_upd_3.png} 
  \caption{Internal representation of the BigText graph of Figure~\ref{fig:BigTextDocs} as a property graph.}
  \label{fig:BigTextStruct}
\end{figure}


\begin{figure}[!t]
  \centering
  \includegraphics[width=3.0in]{figures/scala_2.png}
   \caption{Case classes (in Scala) capturing the BigText-KG as a property graph in Spark's GraphX APIs.
   }
   \label{fig:VertexProp}
\end{figure}
Sentences, clauses and mentions form hierarchical substructures of documents, while links among different mentions (possibly from different clauses or sentences, or even from different documents) to a same entity vertex in the background KB express additional co-references. Recovered implicit relations resulting from apposition (e.g., ``drama'', and ``film'' with respect to ``American Beauty'') and co-reference resolution (``she'' and ``he'' with respect to Thora Birch and Sam Mendes, respectively) are shown as green thin dashed lines in Figure~\ref{fig:BigTextStruct}. Furthermore, the presence of {\em clause} vertices in combination with the disambiguated entity mentions, opens a possibility for a  dynamic extraction of the facts' subgraphs, containing mentions as vertices and the clauses' predicates as labeled edges. Designed in that way, the BigText KG is well suited for the task of RE.

\smallskip
\noindent\textbf{NLP Pipeline.~} Before populating the property graph, documents in the collection are passed through a preconfigured and extensible NLP pipeline which decomposes the input into documents, sentences and clauses. Clauses are generated from sentences with an OIE technique. While each clause represents a semantically coherent block of entity mentions linked by a predicate, mentions first appear in their original lexical form without further linking to typed entities (such as {\tt PER}, {\tt ORG}, {\tt LOC}) or unique knowledge base identifiers, for example WikiData IDs. Therefore, our pipeline also incorporates the steps of Named Entity Recognition (NER) and NamedEntity Disambiguation (NED) as they are available from recent IE tools. Since clauses may have pronouns as their subject and/or object constituents, Coreference Resolution (CR) has been added to the NLP pipeline to increase the coverage of downstream analytical tasks. For example, linking {\em she} in ``... she played Jane Burnham in the highly acclaimed film American Beauty'' to {\em Thora Birch} establishes a connection between the two real-world entities,  ``American Beauty'' and ``Thora Birch'', which can then further be explored. 
\begin{table}[htb]
    \centering
    \small
    \caption{Annotators and background KBs used in the BigText NLP pipeline.}
    \label{tab:annotators}
    \begin{tabular}{|c|c|}
    \hline
    \textbf{Annotation type} & {\textbf{Tools}}  \\
    \hline
    HTML parser & \textbf{Jsoup}\tablefootnote{\scriptsize\url{https://jsoup.org/}} \\
    Tokenization  & Spacy  \\
    OpenIE & \textbf{ClausIE}~\cite{CIE},  \\  
    & OpenIE5\tablefootnote{\scriptsize\url{https://github.com/dair-iitd/OpenIE-standalone}}, \\
    & OpenIE6~\cite{OIE6} \\
    NER & \textbf{StanfordNLP}, \\
    & Flair~\cite{FlairT2021}\\
    NED & \textbf{AIDA-Light}~\cite{aida}, \\
       & REL~\cite{elk_rel}, \\
       & ELQ~\cite{ELQ} \\
    CR & SpanBERT:2018~\cite{LeeSB}, \\
    & SpanBERT:2020~\cite{JoshiSB}\\
     Background & \textbf{YAGO}~\cite{suchanek2007yago}\\
     KB & WikiData\tablefootnote{\scriptsize\url{https://www.wikidata.org/}}\\
    \hline
    \end{tabular}
\end{table} 

Projects which involve the stage of text (pre-) processing typically apply either an entire end-to-end suite of annotation tools, such as NLTK~\cite{bird2009natural}, 
StanfordNLP~\cite{manning2014stanford}, 
SpaCy\footnote{\scriptsize\url{https://spacy.io/}}, or a specific component from it (which can also be substituted with a stand-alone or equivalent tool). Conversely, our text annotation pipeline does not limit the choice of annotators. We intend to use state-of-the-art target-specific components to minimise the risk of error propagation. This strategy allows us to adapt the selection of tools to the type of documents being processed (e.g., long documents corresponding to full-text Wikipedia articles versus short ones, such as Wikipedia articles' abstracts or news). Our implementation also allows for integrating outputs provided by different tools with the same annotation goal. In that way, the pipeline can be configured with further rules that prioritize either precision or recall (e.g., by considering either the intersection or the union of annotations). Table \ref{tab:annotators} depicts the annotation tools that have been integrated into the BigText NLP pipeline so far. 

\smallskip
\noindent\textbf{Applications.~} In the following part of this paper, we focus on {\em relation extraction} (RE) as our main use case application which employs BigText as its underlying knowledge graph and dataset for training Word2Vec model. We use full-text articles of an entire Wikipedia dump from 2019\footnote{\scriptsize\url{https://dumps.wikimedia.org/enwiki/latest/}}. Statistics are shown in Table \ref{tab:graph_stats}. Tools that have been used to process the version discussed here and used for the experiments are shown in Table \ref{tab:annotators} in bold font. 

\begin{table}
  \centering
  \small
  \caption{BigText-KG statistics (in millions) for Wikipedia.}
  \label{tab:graph_stats}
  \begin{tabular}{|ccccc|}
  \hline
  Documents& Sentences& Clauses& Mentions & Entites \\
  \hline
  %5,282,592&97,902,308&190,432,968&283,303,829&2,301,513\\
  5.3 & 97 &190 &283 &2 \\
  \hline
  \end{tabular}
\end{table} 

